$k$FW: A Frank-Wolfe style algorithm with stronger subproblem oracles

This paper proposes a new variant of Frank-Wolfe (FW), called $k$FW. Standard FW suffers from slow convergence: iterates often zig-zag as update directions oscillate around extreme points of the constraint set. The new variant, $k$FW, overcomes this problem by using two stronger subproblem oracles in each iteration. The first is a $k$ linear optimization oracle ($k$LOO) that computes the $k$ best update directions (rather than just one). The second is a $k$ direction search ($k$DS) that minimizes the objective over a constraint set represented by the $k$ best update directions and the previous iterate. When the problem solution admits a sparse representation, both oracles are easy to compute, and $k$FW converges quickly for smooth convex objectives and several interesting constraint sets: $k$FW achieves finite $\frac{4L_f^3D^4}{\gamma\delta^2}$ convergence on polytopes and group norm balls, and linear convergence on spectrahedra and nuclear norm balls. Numerical experiments validate the effectiveness of $k$FW and demonstrate an order-of-magnitude speedup over existing approaches.

==> defs.tex <==
% Notes
%\usepackage[usenames,dvipsnames]{xcolor}
%\definecolor{purple}{rgb}{0.3,0.0,.4}
\newcommand{\mnote}[1]{\textcolor{black}{\textbf{[MU: #1]}}}
\newcommand{\lnote}[1]{\textcolor{red}{\textbf{[LD: #1]}}}
\newcommand{\jatnote}[1]{\textcolor{blue}{\textbf{[JAT: #1]}}}
%\renewcommand{\mnote}[1]{}
%\renewcommand{\lnote}[1]{}
\renewcommand{\jatnote}[1]{}


% for restatement of lemmas and theorems
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}
\usepackage{xspace}
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\declaretheorem[name=Theorem,numberwithin=section]{thm}
% some traditional defintions that can be blamed on craig barratt
\newcommand{\defn}{:\,=}
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}

% text abbrevs

%%% Modern composition rules set these Latin abbreviations in roman text.
%%% Exempli gratia and id est have a comma afterward.
%%% cf. The Chicago Manual of Style.

\newcommand{\cf}{cf.}
\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}

\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\posint}{{\mbox{\bf N}}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{{\mbox{\bf C}}}
\newcommand{\sym}{{\mbox{\bf S}}}  % symmetric matrices

% lin alg stuff
\newcommand{\Span}{\mathop{\bf span}}
\newcommand{\range}{\mathop{\bf range}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\nullspace}{{\mathop {\bf null}}}
\newcommand{\tr}{\mathop{\bf tr}}
\newcommand{\Tr}{\mathop{\bf tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}
\newcommand{\ms}{\mathop{\bf MaxSingVec}}

% norm
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{\mbox{\tiny{F}}}}
\newcommand{\opnorm}[1]{\left\|#1\right\|_{\mbox{\tiny{\textup{op}}}}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\arbnorm}[1]{\left\|#1\right\|_\alpha}
\newcommand{\darbnorm}[1]{\left\|#1\right\|^*_\alpha}
% probability stuff
\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}
\newcommand{\sign}{\mathop{\bf sign}}

% convexity & optimization stuff
\newcommand{\Co}{{\mathop {\bf Co}}}
\newcommand{\co}{{\mathop {\bf Co}}}
\newcommand{\Var}{\mathop{\bf var{}}}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}
%\renewcommand{\QED}{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\epi}{\mathop{\bf epi}}
%\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\var}{\mathop{\bf var}}
\newcommand{\Card}{\mathop{\bf card}}
\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bd}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\xopt}{x^{\rm opt}}
\newcommand{\prox}{{\bf prox}}
\newcommand{\conj}{{\bf conj}}
\newcommand{\update}{\mathop{\bf update}}
\newcommand{\indicator}{{\bf 1}}

% for statistics
\newcommand{\huber}{\mathop{\bf huber}}
\newcommand{\sort}{\mathop{\bf sort}}
\newcommand{\round}{\mathop{\bf round}}


% for prettiness
\newcommand{\half}{(1/2)}

% for constants
\newcommand{\constanta}{\frac{\sigma_{\min}(\mathcal{A}_{V^\star})}{4\|\mathcal{A}\|_{op}}}
\newcommand{\constantb}{\frac{2\cdot \constanta \lambda_{\min>0}(Z^\star)}{4\frac{1}{\sigma_{\min}(\mathcal{D})}\sqrt{1+4\cdot \constanta}+1}}
\newcommand{\constantc}{\frac{2\cdot \constantb\lambda_{\min>0}(X^\star)}{\sqrt{4\|Z^\star\|_{op}+4\constantb}+4\|Z^\star\|_{op}}}
\newcommand{\constantd}{\frac{\lambda^2_{n-r}(Z^\star)}{\frac{1}{\sigma^2_{\min}(\mathcal{D})}(4\sqrt{\|Z^\star\|_{op}}+2\sqrt{ \frac{\lambda_{n-r}(Z^\star)}{\frac{1}{\sigma_{\min}(\mathcal{D})}}})^2}\lambda_{\min >0}(X^\star)}
\newcommand{\constante}{ \frac{\lambda_{\min>0}(X^\star)\|Z^\star\|_{op}}{10(\frac{1}{\sigma_{\min}(\mathcal{D})}+\frac{1}{\sigma^2_{\min}(\mathcal{D})}}}
\newcommand{\constantA}{\frac{\delta_S}{\sigma_{\min}(\mathcal{A}_V)} +\opnorm{S}}
\newcommand{\constantD}{\frac{\constantE}{1+\kappa_V}}
\newcommand{\constantE}{\phi}
\newcommand{\constantB}{\frac{1}{4}\biggr[ \sqrt{2\constantE^2+4\biggr(\constantA\biggr) +4\constantD}+\sqrt{2}\constantE\biggr]^2}

%% theorems
%\theoremstyle{definition} % don't italicize theorems
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{prop}{Proposition}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%% alg description --- not much for now!
%\newenvironment{algdesc}%
%{\begin{quote}}{\end{quote}}
%
%% figures
%\def\figbox#1{\framebox[\hsize]{\hfil\parbox{0.9\hsize}{#1}}}
%% figure size
%\makeatletter
%\newlength \figwidth
%\if@twocolumn
%  \setlength \figwidth {0.9\columnwidth}
%\else
%  \setlength \figwidth {0.5\textwidth}
%\fi
%\makeatother

% \showthe\figwidth

% captions a la sirev
%\makeatletter
%\long\def\@makecaption#1#2{
%   \vskip 9pt
%   \begin{small}
%   \setbox\@tempboxa\hbox{{\bf #1:} #2}
%   \ifdim \wd\@tempboxa > 5.5in
%        \begin{center}
%        \begin{minipage}[t]{5.5in}
%        \addtolength{\baselineskip}{-0.95pt}
%        {\bf #1:} #2 \par
%        \addtolength{\baselineskip}{0.95pt}
%        \end{minipage}
%        \end{center}
%   \else
%	\hbox to\hsize{\hfil\box\@tempboxa\hfil}
%   \fi
%   \end{small}\par
%}
%\makeatother

%bigO
\newcommand{\bigO}[1]{\mathcal{O}(#1)}

%for SDP slackness project
\newcommand{\pval}{p_\star}
\newcommand{\dval}{d_\star}
\newcommand{\dm}{n}
\newcommand{\cons}{m}
\newcommand{\rsol}{r_\star}
\newcommand{\xsol}{X_\star}
\newcommand{\ysol}{y_\star}
\newcommand{\zsol}{Z(\ysol)}%{Z_\star}
\newcommand{\hsol}{h_\star }
\newcommand{\ssol}{S_\star}
\newcommand{\xsolset}{\mathcal{X}_\star}

\newcommand{\vspacex}{\mathcal{V}_\star}
\newcommand{\uspacex}{\mathcal{U}_\star}

%\newcommand{\vspacex}{\mathcal{V}_\star(\xsol)}
%\newcommand{\uspacex}{\mathcal{U}_\star(\zsol)}

\newcommand{\vrepx}{V_\star(\xsol)}
\newcommand{\urepx}{U_\star(\zsol)}
\newcommand{\vspaceox}{\mathcal{V}_\star}
\newcommand{\uspaceox}{\mathcal{U}_\star}
\newcommand{\vrepox}{{V_\star}}
\newcommand{\urepox}{{U_\star}}
\newcommand{\scmu}{\mu_{\mathcal{SC}}}
\newcommand{\infeasx}{X_{\textup{infeas}}}
\newcommand{\objx}{X_{\text{obj}}}
\newcommand{\objp}{g_\alpha}
\newcommand{\objc}{C}
\newcommand{\Amap}{\mathcal{A}}
\newcommand{\bvec}{b}
\newcommand{\cond}{\kappa}
\newcommand{\Av}[1]{\Amap_{#1}}
\newcommand{\Admap}{\mathcal{A}^*}
\newcommand{\ineqov}[1]{\overset{#1}{\leq}}
\newcommand{\alg}{\mathcal{G}}
\newcommand{\accelgrad}{\textbf{AccelGrad}\xspace}
\newcommand{\adangd}{\textbf{AdaNGD}\xspace}
\newcommand{\adagrad}{\textbf{AdaGrad}\xspace}
\newcommand{\unipd}{\textbf{UniPD}}
\newcommand{\trux}{\bar{X}}
%matrix completion
\newcommand{\projomega}{\Pi_{\Omega}}

%problem name
\newcommand{\minfeas}{MinFeasSDP\xspace}
\newcommand{\minobj}{MinObjSDP\xspace}

